A new class of finite element variational multiscale turbulence models for incompressible magnetohydrodynamics

New large eddy simulation (LES) turbulence models for incompressible magnetohydrodynamics (MHD) derived from the variational multiscale (VMS) formulation for finite element simulations are introduced. The new models include the variational multiscale formulation, a residual-based eddy viscosity model, and a mixed model that combines both of these component models. Each model contains terms that are proportional to the residual of the incompressible MHD equations and is therefore numerically consistent. Moreover, each model is also dynamic, in that its effect vanishes when this residual is small. The new models are tested on the decaying MHD Taylor Green vortex at low and high Reynolds numbers. The evaluation of the models is based on comparisons with available data from direct numerical simulations (DNS) of the time evolution of energies as well as energy spectra at various discrete times. A numerical study, on a sequence of meshes, is presented that demonstrates that the large eddy simulation approaches the DNS solution for these quantities with spatial mesh refinement.

==> Bibliography.tex <==
\begin{thebibliography}{10}

\bibitem{aluie2010scale}
H.~Aluie and G.~L. Eyink.
\newblock Scale locality of magnetohydrodynamic turbulence.
\newblock {\em Physical review letters}, 104:81101, 2010.

\bibitem{badia2013unconditionally}
Santiago Badia, Ramon Codina, and Ramon Planas.
\newblock On an unconditionally convergent stabilized finite element
  approximation of resistive magnetohydrodynamics.
\newblock {\em Journal of Computational Physics}, 234:399--416, 2013.

\bibitem{baerenzung2008spectrala}
J.~Baerenzung, H.~Politano, Y.~Ponty, and A.~Pouquet.
\newblock Spectral modeling of magnetohydrodynamic turbulent flows.
\newblock {\em Physical Review E}, 78:026310, 2008.

\bibitem{batchelor1982theory}
G.~K. Batchelor.
\newblock {\em The Theory of Homogeneous Turbulence}.
\newblock Cambridge: Cambridge University Press, 1982.

\bibitem{bazilevs2007variational}
Y.~Bazilevs, V.M. Calo, J.A. Cottrell, T.J.R. Hughes, A.~Reali, and
  G.~Scovazzi.
\newblock Variational multiscale residual-based turbulence modeling for large
  eddy simulation of incompressible flows.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  197:173--201, 2007.

\bibitem{beresnyak2011spectral}
A.~Beresnyak.
\newblock Spectral slope and kolmogorov constant of mhd turbulence.
\newblock {\em Physical Review Letters}, 106:75001, 2011.

\bibitem{biskamp2003magnetohydrodynamic}
D.~Biskamp.
\newblock {\em Magnetohydrodynamic Turbulence}.
\newblock Cambridge: Cambridge University Press, 2003.

\bibitem{brooks1982streamline}
Alexander~N Brooks and Thomas~JR Hughes.
\newblock Streamline upwind/petrov-galerkin formulations for convection
  dominated flows with particular emphasis on the incompressible navier-stokes
  equations.
\newblock {\em Computer methods in applied mechanics and engineering},
  32(1):199--259, 1982.

\bibitem{codina2002stabilized}
R.~Codina.
\newblock Stabilized finite element approximation of transient incompressible
  flows using orthogonal subscales.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  191:4295--4321, 2002.

\bibitem{codina2006stabilized}
R.~Codina and N.~Hern\'{a}ndez-Silva.
\newblock Stabilized finite element approximation of the stationary
  magneto-hydrodynamics equations.
\newblock {\em Computational Mechanics}, 38:344--355, 2006.

\bibitem{codina2007time}
R.~Codina, J.~Principe, O.~Guasch, and S.~Badia.
\newblock Time dependent subscales in the stabilized finite element
  approximation of incompressible flow problems.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  196:2413--2430, 2007.

\bibitem{dallas2013origins}
V.~Dallas and A.~Alexakis.
\newblock The origins of {$k^{-2}$} spectrum in the decaying taylor-green
  magnetohydrodynamic turbulent flows.
\newblock {\em Phys. Rev. E}, 88:053014, Nov 2013.

\bibitem{davidson2001introduction}
P.A. Davidson.
\newblock {\em An Introduction to Magnetohydrodynamics}, volume~25.
\newblock New York: Cambridge University Press, 2001.

\bibitem{franca1992stabilized}
Leopoldo~P Franca, Sergio~L Frey, and Thomas~JR Hughes.
\newblock Stabilized finite element methods: I. application to the
  advective-diffusive model.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  95(2):253--276, 1992.

\bibitem{gerbeau2000stabilized}
J-F Gerbeau.
\newblock A stabilized finite element method for the incompressible
  magnetohydrodynamic equations.
\newblock {\em Numerische Mathematik}, 87(1):83--111, 2000.

\bibitem{germano1991dynamic}
M.~Germano, U.~Piomelli, P.~Moin, and W.~H. Cabot.
\newblock A dynamic subgrid-scale eddy viscosity model.
\newblock {\em Physics of Fluids A: Fluid Dynamics}, 3:1760, 1991.

\bibitem{goedbloed2010advanced}
H.~Goedbloed, R.~Keppens, and S.~Poedts.
\newblock {\em Advanced Magnetohydrodynamics}, volume~1.
\newblock New York: Cambridge University Press, 2010.

\bibitem{goedbloed2006principles}
H.~Goedbloed and S.~Poedts.
\newblock {\em Principles of Magnetohydrodynamics}, volume~74.
\newblock New York: Cambridge University Press, 2006.

\bibitem{haugen2006hydrodynamic}
N.E. Haugen and A.~Brandenburg.
\newblock Hydrodynamic and hydromagnetic energy spectra from large eddy
  simulations.
\newblock {\em Physics of Fluids}, 18:075106, 2006.

\bibitem{holm2002lagrangian}
D.D. Holm.
\newblock Lagrangian averages, averaged lagrangians, and the mean effects of
  fluctuations in fluid dynamics.
\newblock {\em Chaos: An Interdisciplinary Journal of Nonlinear Science},
  12:518--530, 2002.

\bibitem{hughes2000large}
Thomas~JR Hughes, Luca Mazzei, and Kenneth~E Jansen.
\newblock Large eddy simulation and the variational multiscale method.
\newblock {\em Computing and Visualization in Science}, 3(1-2):47--59, 2000.

\bibitem{hughes1995multiscale}
T.J.R. Hughes.
\newblock Multiscale phenomena: Green's functions, the dirichlet-to-neumann
  formulation, subgrid scale models, bubbles and the origins of stabilized
  methods.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  127:387--401, 1995.

\bibitem{hughes2000finite}
T.J.R. Hughes.
\newblock {\em The Finite Element Method: Linear Static and Dynamic Finite
  Element Analysis}.
\newblock Mineola, New York: Dover Publications, 2000.

\bibitem{hughes1998variational}
T.J.R. Hughes, G.R. Feij{\'o}o, L.~Mazzei, and J.B. Quincy.
\newblock The variational multiscale method--a paradigm for computational
  mechanics.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  166:3--24, 1998.

\bibitem{hughes1986new}
T.J.R. Hughes, L.~P. Franca, and M.~Balestra.
\newblock A new finite element formulation for computational fluid dynamics: V.
  circumventing the babu{\v{s}}ka-brezzi condition: A stable petrov-galerkin
  formulation of the stokes problem accommodating equal-order interpolations.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  59:85--99, 1986.

\bibitem{hughes1989new}
T.J.R. Hughes, L.P. Franca, and G.M. Hulbert.
\newblock A new finite element formulation for computational fluid dynamics:
  Viii. the galerkin/least-squares method for advective-diffusive equations.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  73:173--189, 1989.

\bibitem{hughes2008variational}
T.J.R. Hughes and G.~Sangalli.
\newblock Variational multiscale analysis: The fine-scale green's function,
  projection, optimization, localization, and stabilized methods.
\newblock {\em SIAM Journal on Numerical Analysis}, 45:539--557, 2008.

\bibitem{knaepen2004large}
B.~Knaepen and P.~Moin.
\newblock Large-eddy simulation of conductive flows at low magnetic reynolds
  number.
\newblock {\em Physics of Fluids}, 16:1255, 2004.

\bibitem{kraichnan1976eddy}
R.H. Kraichnan.
\newblock Eddy viscosity in two and three dimensions.
\newblock {\em Journal of Atmospheric Science}, 33(8):1521--1536, 1976.

\bibitem{lee2010lack}
E.~Lee, M.E. Brachet, A.~Pouquet, P.D. Mininni, and D.~Rosenberg.
\newblock Lack of universality in decaying magnetohydrodynamic turbulence.
\newblock {\em Physical Review E}, 81:016318, 2010.

\bibitem{muller2002large}
W.C.. M\"{u}ller and D.~Carati.
\newblock Large-eddy simulation of magnetohydrodynamic turbulence.
\newblock {\em Computer Physics Communications}, 147:544--547, 2002.

\bibitem{oberai2014residual}
A.A. Oberai, J.~Lui, D.~Sondak, and T.J.R. Hughes.
\newblock A residual-based eddy viscosity model for the les of turbulent flows.
\newblock {\em Comput. Methods Appl. Mech. Engrg.}, 2014.

\bibitem{oberai2011application}
A.A. Oberai and D.~Sondak.
\newblock Application of the variational germano identity to the variational
  multiscale formulation.
\newblock {\em International Journal for Numerical Methods in Biomedical
  Engineering}, 27:335--344, 2011.

\bibitem{oberai2005dynamic}
A.A. Oberai and J.~Wanderer.
\newblock A dynamic approach for evaluating parameters in a numerical method.
\newblock {\em International Journal for Numerical Methods in Engineering},
  62:50--71, 2005.

\bibitem{peyret2010spectral}
R.~Peyret.
\newblock {\em Spectral Methods for Incompressible Viscous Flow}.
\newblock New York: Springer-Verlag New York, Inc, 2010.

\bibitem{ponty2004simulation}
Y.~Ponty, H.~Politano, and J-F.~P. Pinton.
\newblock Simulation of induction at low magnetic prandtl number.
\newblock {\em Physical Review Letters}, 92:144503, 2004.

\bibitem{pope2000turbulent}
S.~B. Pope.
\newblock {\em Turbulent Flows}.
\newblock New York: Cambridge University Press, 2000.

\bibitem{pouquet2010dynamics}
A.~Pouquet, E.~Lee, M.E. Brachet, P.D. Mininni, and D.~Rosenberg.
\newblock The dynamics of unforced turbulence at high reynolds number for
  taylor--green vortices generalized to mhd.
\newblock {\em Geophysical and Astrophysical Fluid Dynamics}, 104:115--134,
  2010.

\bibitem{rogallo1984numerical}
Robert~S Rogallo and Parviz Moin.
\newblock Numerical simulation of turbulent flows.
\newblock {\em Annual Review of Fluid Mechanics}, 16(1):99--137, 1984.

\bibitem{sagaut2002large}
Pierre Sagaut.
\newblock {\em Large eddy simulation for incompressible flows}.
\newblock Springer, 2002.

\bibitem{schmidt2014large}
Wolfram Schmidt.
\newblock Large eddy simulations in astrophysics.
\newblock {\em arXiv preprint arXiv:1404.2483}, 2014.

\bibitem{shadid2010towards}
J.N. Shadid, R.P. Pawlowski, J.W. Banks, L.~Chacon, P.T. Lin, and R.S.
  Tuminaro.
\newblock Towards a scalable fully-implicit fully-coupled resistive {MHD} formulation with stabilized {FE} methods.
\newblock {\em Journal of Computational Physics}, 229:7649--7671, 2010.

\bibitem{shadidetalMHD_2013}
J.N. Shadid, R.P. Pawlowski, E. C. Cyr, R. S. Tuminaro, L.~Chacon, and P. D. Weber.
\newblock Scalable Implicit Incompressible  Resistive {MHD} with Stabilized FE  and Fully-coupled Newton-Krylov-AMG.
\newblock {\em in preparation}, 2014.

\bibitem{sondak2012large}
D.~Sondak and A.A. Oberai.
\newblock Large eddy simulation models for incompressible magnetohydrodynamics
  derived from the variational multiscale formulation.
\newblock {\em Physics of Plasmas}, 19:102308, 2012.

\bibitem{tezduyar1991stabilized}
Tayfun~E Tezduyar.
\newblock Stabilized finite element formulations for incompressible flow
  computations.
\newblock {\em Advances in applied mechanics}, 28:1--44, 1991.

\bibitem{theobald1994subgrid}
M.L. Theobald, P.A. Fox, and S.~Sofia.
\newblock A subgrid-scale resistivity for magnetohydrodynamics.
\newblock {\em Physics of Plasmas}, 1:3016, 1994.

\bibitem{wang2010spectral}
Z.~Wang and A.A. Oberai.
\newblock Spectral analysis of the dissipation of the residual-based
  variational multiscale method.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  199:810--818, 2010.

\bibitem{yoshizawa1991subgrid}
A.~Yoshizawa.
\newblock Subgrid-scale modeling of magnetohydrodynamic turbulence.
\newblock {\em Physical Society of Japan}, 60:9--12, 1991.

\bibitem{Dennis-Schnabel}
 Dennis, Jr., J. E. and R. B. Schnabel.
\newblock Numerical Methods for Unconstrained Optimization and Nonlinear Equations.
 \newblock Prentice-Hall, Series in Automatic Computation , 1983.

\bibitem{EW94}
S. C. Eisenstat and H. F. Walker.
 \newblock  Globally convergent inexact {N}ewton methods.
 \newblock SIAM J. Optimization, 4, 393-422, 1994.

\bibitem{EW96}
S. C. Eisenstat and H. F. Walker.
 \newblock  Choosing the forcing terms in an inexact {N}ewton method.
 \newblock  SIAM J. Sci. Comput., 17,16-32,1996. 

\bibitem{tuminaro-cnme}
R.S. Tuminaro, C.H. Tong, J.N. Shadid, K.D.Devine and D.M. Day
 \newblock  On a multilevel preconditioning module for unstructured mesh {Krylov} solvers: two-level {Schwarz}.
  \newblock  Comm. Num. Method. Eng., 002, 18, 383-389.

\bibitem{shadid2004}
 J.N. Shadid, R.S. Tuminaro, K.D. Devine, G.L. Henningan and P.T. Lin.
 \newblock  Performance of fully-coupled domain decomposition preconditioners for finite element transport/reaction simulations.
 \newblock  J. Comput. Phys., 205, 1", 24-47, 2005.


\bibitem{Shadid2006}
J. N. Shadid, A. G. Salinger, R. P. Pawlowski,  P. T. Lin, G. L. Hennigan, R. S. Tuminaro and R. B. Lehoucq.
  \newblock   Stabilized {FE} Computational Analysis of Nonlinear Steady State Transport/Reaction Systems.
  \newblock  Comp. Meth. Applied Mech. Eng, 195, 1846-1871, 2006."

@article{lin2010AMGjcp}
 P. T. Lin, J. N. Shadid, R. S. Tuminaro, M. Sala, G. L. Hennigan and R. P. Pawlowski.
  \newblock   A Parallel Fully-Coupled Algebraic Multilevel Preconditioner Applied to Multiphysics {PDE} Applications: Drift-diffusion, Flow/transport/reaction, Resistive {MHD}. 
  \newblock   Int. J. Num. Meth. Fluids, 2010, 64, 1148-1179


\end{thebibliography}
